Bounded Rationality in Concurrent Parity Games

We consider 2-player games played on a finite state space for infinite rounds. The games are concurrent: in each round, the two players choose their moves simultaneously; the current state and the moves determine the successor. We consider omega-regular winning conditions given as parity objectives. We consider the qualitative analysis problems: the computation of the almost-sure and limit-sure winning set of states, where player 1 can ensure to win with probability 1 and with probability arbitrarily close to 1, respectively. In general the almost-sure and limit-sure winning strategies require both infinite-memory and infinite-precision. We study the bounded-rationality problem for qualitative analysis of concurrent parity games, where the strategy set player 1 is restricted to bounded-resource strategies. In terms of precision, strategies can be deterministic, uniform, finite-precision or infinite-precision; and in terms of memory, strategies can be memoryless, finite-memory or infinite-memory. We present a precise and complete characterization of the qualitative winning sets for all combinations of classes of strategies. In particular, we show that uniform memoryless strategies are as powerful as finite-precision infinite-memory strategies, and infinite-precision memoryless strategies are as powerful as infinite-precision finite-memory strategies. We show that the winning sets can be computed in O(n^{2d+3}) time, where n is the size of the game and 2d is the number of priorities, and our algorithms are symbolic. The membership problem of whether a state belongs to a winning set can be decided in NP cap coNP. While this complexity is the same as for the simpler class of turn-based games, where in each state only one of the players has a choice of moves, our algorithms, that are obtained by characterization of the winning sets as mu-calculus formulas, are considerably more involved.

==> check <==
This is pdfeTeXk, Version 3.141592-1.21a-2.2 (Web2C 7.5.4)
 file:line:error style messages enabled.
 %&-line parsing enabled.
entering extended mode
(./main.tex
LaTeX2e <2003/12/01>
Babel <v3.8d> and hyphenation patterns for american, french, german, ngerman, b
ahasa, basque, bulgarian, catalan, croatian, czech, danish, dutch, esperanto, e
stonian, finnish, greek, icelandic, irish, italian, latin, magyar, norsk, polis
h, portuges, romanian, russian, serbian, slovak, slovene, spanish, swedish, tur
kish, ukrainian, nohyphenation, loaded.
(/usr/share/texmf/tex/latex/base/article.cls
Document Class: article 2004/02/16 v1.4f Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size11.clo))
(/usr/share/texmf/tex/latex/base/latexsym.sty)
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsfonts/amssymb.sty
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf/tex/latex/preprint/fullpage.sty) (./epsfig.sty
Document style option `epsfig', v1.20 <26.1.94> (edited by SPQR)
(/usr/share/texmf/tex/generic/epsf/epsf.tex
This is `epsf.tex' v2.7k <10 July 1997>
)) (./eepic.sty
Extension to Epic and LaTeX. Version 1.1e - Released Dec 21, 1999
) (./gastex.sty (/usr/share/texmf/tex/latex/tools/calc.sty)
(/usr/share/texmf/tex/latex/graphics/trig.sty)) (./luca.sty)
(/usr/share/texmf/tex/latex/psnfss/times.sty) (./main.aux)
(/usr/share/texmf/tex/latex/psnfss/ot1ptm.fd)
(/usr/share/texmf/tex/latex/base/ulasy.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsb.fd)
(/usr/share/texmf/tex/latex/psnfss/ot1pcr.fd) [1] [2] [3]

LaTeX Warning: Reference `examp-counter-almost' on page 4 undefined on input li
ne 566.

[4] (./definitions.tex (/usr/share/texmf/tex/latex/psnfss/omsptm.fd)
Underfull \hbox (badness 1783) in paragraph at lines 93--100
\OT1/ptm/b/n/10.95 Equivalent game struc-tures. \OT1/ptm/m/n/10.95 Given two ga
me struc-tures $\OMS/cmsy/m/n/10.95 G[] \OT1/cmr/m/n/10.95 = \OMS/cmsy/m/n/10.9
5 h\OML/cmm/m/it/10.95 S; []; \OT1/cmr/m/n/10.95 ^^@[]\OML/cmm/m/it/10.95 ; \OT
1/cmr/m/n/10.95 ^^@[]\OML/cmm/m/it/10.95 ; ^^N[]\OMS/cmsy/m/n/10.95 i$ \OT1/ptm
/m/n/10.95 and $\OMS/cmsy/m/n/10.95 G[] \OT1/cmr/m/n/10.95 =
[5] [6]
Underfull \hbox (badness 3229) in paragraph at lines 352--358
[]\OT1/ptm/m/n/10.95 Given a set $\OML/cmm/m/it/10.95 U \OMS/cmsy/m/n/10.95 ^^R
 \OML/cmm/m/it/10.95 S$ \OT1/ptm/m/n/10.95 we use usual LTL no-ta-tions $\U/las
y/m/n/10.95 2\OML/cmm/m/it/10.95 U; \U/lasy/m/n/10.95 3\OML/cmm/m/it/10.95 U; \
U/lasy/m/n/10.95 23\OML/cmm/m/it/10.95 U$ \OT1/ptm/m/n/10.95 and $\U/lasy/m/n/1
0.95 32\OML/cmm/m/it/10.95 U$ \OT1/ptm/m/n/10.95 to de-note
[7] [8]) (./pure.tex [9] [10] [11]
Underfull \hbox (badness 4096) in paragraph at lines 231--248
\OT1/ptm/b/n/10.95 Computation of $[][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 
U; M; \OT1/cmr/m/n/10.95 ^^H)$\OT1/ptm/b/n/10.95 . \OT1/ptm/m/n/10.95 It fol-lo
ws from Propo-si-tion 2[] that the com-pu-ta-tion of
(./big-proof1.tex [12] [13] [14]
Underfull \hbox (badness 2111) in paragraph at lines 230--236
[]\OT1/ptm/m/it/10.95 Observe that if the pred-i-cate $[][]\OT1/cmr/m/n/10.95 (
\OML/cmm/m/it/10.95 Y[]\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m/it/10.95 is re-moved fr
om the pre-de-ces-sor op-er-a-tor

Underfull \hbox (badness 10000) in paragraph at lines 230--236
[][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X[]\OT1/cmr/
m/n/10.95 )$ \OT1/ptm/m/it/10.95 (resp. $[][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/
10.95 i; Y[]; X[]; [] ; Y[]; X[]; Y[]\OT1/cmr/m/n/10.95 )$\OT1/ptm/m/it/10.95 )
,

Underfull \hbox (badness 10000) in paragraph at lines 230--236
\OT1/ptm/m/it/10.95 then we ob-tain the op-er-a-tor $[][]\OT1/cmr/m/n/10.95 (\O
ML/cmm/m/it/10.95 i \OMS/cmsy/m/n/10.95 ^^@ \OT1/cmr/m/n/10.95 1\OML/cmm/m/it/1
0.95 ; X[]; Y[]; [] ; X[]; Y[]; X[]\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m/it/10.95 (r
esp.

Overfull \hbox (4.46823pt too wide) detected at line 272
\OML/cmm/m/it/10.95 ^^WY[]:^^VX[]:^^WY[]:^^VX[]: [] ^^WY[]:^^VX[]:^^WY[]: []
[15]
Overfull \hbox (12.87668pt too wide) detected at line 306
\OML/cmm/m/it/10.95 ^^VY[]:^^WX[]:^^VY[]:^^WX[]: [] ^^VY[]:^^WX[]:^^VY[]: []
[16] [17] [18] [19]
Overfull \hbox (21.4319pt too wide) detected at line 717
[]

Underfull \hbox (badness 1675) in paragraph at lines 726--730
[]  []\OT1/ptm/m/it/10.95 For a par-ity func-tion $\OML/cmm/m/it/10.95 p \OT1/c
mr/m/n/10.95 : \OML/cmm/m/it/10.95 S \OMS/cmsy/m/n/10.95 7! \OT1/cmr/m/n/10.95 
[0\OML/cmm/m/it/10.95 ::\OT1/cmr/m/n/10.95 2\OML/cmm/m/it/10.95 n\OT1/cmr/m/n/1
0.95 ]$\OT1/ptm/m/it/10.95 , and for all $\OML/cmm/m/it/10.95 T \OMS/cmsy/m/n/1
0.95 ^^R \OML/cmm/m/it/10.95 S$\OT1/ptm/m/it/10.95 , we have $\OML/cmm/m/it/10.
95 W \OMS/cmsy/m/n/10.95 ^^R
[20] [21]
Overfull \hbox (2.68309pt too wide) detected at line 865
\OML/cmm/m/it/10.95 ^^WX[]:^^VY[]:^^WX[]: [] ^^VY[]:^^WX[]:^^VY[]: []
[22]
Overfull \hbox (8.2834pt too wide) detected at line 990
\OML/cmm/m/it/10.95 W \OT1/cmr/m/n/10.95 = \OML/cmm/m/it/10.95 ^^VX[]:^^WY[]:^^
VX[]: [] ^^WY[]:^^VX[] [] :
[23] [24]
Overfull \hbox (8.098pt too wide) detected at line 1159
\OML/cmm/m/it/10.95 ^^VY[]:^^WX[]:^^VY[]:^^WX[]: [] ^^VY[]:^^WX[] []
[25] [26] [27]
Overfull \hbox (8.098pt too wide) detected at line 1321
\OML/cmm/m/it/10.95 ^^VY[]:^^WX[]:^^VY[]:^^WX[]: [] ^^VY[]:^^WX[] []
[28] [29] (./dual-pre-uniform.tex
Underfull \hbox (badness 10000) in paragraph at lines 26--32
[]\OT1/ptm/m/it/10.95 For all $\OML/cmm/m/it/10.95 s \OMS/cmsy/m/n/10.95 2 \OML
/cmm/m/it/10.95 S$\OT1/ptm/m/it/10.95 , if $\OML/cmm/m/it/10.95 s \OMS/cmsy/m/n
/10.95 2 [][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X[]
\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m/it/10.95 (resp. $\OML/cmm/m/it/10.95 s \OMS/cm
sy/m/n/10.95 2

Underfull \hbox (badness 10000) in paragraph at lines 26--32
[][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X[]; Y[]\OT1
/cmr/m/n/10.95 )$\OT1/ptm/m/it/10.95 ), then there ex-ists uni-form dis-tri-bu-


Underfull \hbox (badness 10000) in paragraph at lines 26--32
\OT1/ptm/m/it/10.95 tion $\OML/cmm/m/it/10.95 ^^X[]$ \OT1/ptm/m/it/10.95 to wit
-ness that $\OML/cmm/m/it/10.95 s \OMS/cmsy/m/n/10.95 2 [][]\OT1/cmr/m/n/10.95 
(\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X[]\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m
/it/10.95 (resp. $\OML/cmm/m/it/10.95 s \OMS/cmsy/m/n/10.95 2
[30] [31] [32])) [33] [34]
Underfull \hbox (badness 6842) in paragraph at lines 514--519
[] \OT1/ptm/b/n/10.95 ($[][]\OT1/cmr/m/n/10.95 ([]\OML/cmm/m/it/10.95 ; []; \OT
1/cmr/m/n/10.95 ^^H) \U/msb/m/n/10.95 ( [][]\OT1/cmr/m/n/10.95 ([]\OML/cmm/m/it
/10.95 ; []; \OT1/cmr/m/n/10.95 ^^H)$\OT1/ptm/b/n/10.95 ).  []\OT1/ptm/m/n/10.9
5 We show with an ex-am-ple that
[35]) (./limit-finite.tex [36] [37]
Overfull \hbox (13.0226pt too wide) in paragraph at lines 342--345
 [] 
[38] (./big-proof2.tex [39] [40] [41]
Underfull \hbox (badness 3668) in paragraph at lines 196--201
[]\OT1/ptm/m/it/10.95 Observe that if we rule out the pred-i-cate $[][]\OT1/cmr
/m/n/10.95 (\OML/cmm/m/it/10.95 X[]; Y[]\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m/it/10.
95 the pre-de-ces-sor op-er-a-tor

Underfull \hbox (badness 3701) in paragraph at lines 196--201
\OT1/ptm/m/it/10.95 then we ob-tain the sim-pler pre-de-ces-sor op-er-a-tor $[]
[]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 i; X[]; Y[]; [] ; Y[]; X[]\OT1/cmr/m/
n/10.95 )$ \OT1/ptm/m/it/10.95 (resp.
(./formal-limit-pre.tex [42] [43]) [44] [45]
Underfull \hbox (badness 10000) in paragraph at lines 392--401
\OT1/ptm/b/n/10.95 Claim. \OT1/ptm/m/n/10.95 We show that for $\OML/cmm/m/it/10
.95 X[] \OMS/cmsy/m/n/10.95 ^^R \OML/cmm/m/it/10.95 X[] \OMS/cmsy/m/n/10.95 ^^R
 \OML/cmm/m/it/10.95 Y[] \OMS/cmsy/m/n/10.95 ^^R \OML/cmm/m/it/10.95 Y[]$ \OT1/
ptm/m/n/10.95 we have
[46] [47] (./gen.tex
Overfull \hbox (6.37802pt too wide) detected at line 28
[]
[48]
Overfull \hbox (18.19014pt too wide) in paragraph at lines 58--86
[]\OT1/ptm/m/n/10.95 We first show that if $[][] \OT1/cmr/m/n/10.95 = ^^@[](\OM
L/cmm/m/it/10.95 s\OT1/cmr/m/n/10.95 )$\OT1/ptm/m/n/10.95 , then $\OML/cmm/m/it
/10.95 s \OMS/cmsy/m/n/10.95 2 [][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 Y[];
 X[]\OT1/cmr/m/n/10.95 )  []  [][](\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X
[]\OT1/cmr/m/n/10.95 )$\OT1/ptm/m/n/10.95 .
[49]
Overfull \hbox (13.0751pt too wide) detected at line 186
[]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 s; a[]; b\OT1/cmr/m/n/10.95 ) \OMS/cm
sy/m/n/10.95 ^^R :\OML/cmm/m/it/10.95 X[] \OMS/cmsy/m/n/10.95 ^ 9\OT1/cmr/m/n/1
0.95 0 \OMS/cmsy/m/n/10.95 ^^T \OML/cmm/m/it/10.95 j \OMS/cmsy/m/n/10.95 ^^T \O
ML/cmm/m/it/10.95 i:\OT1/cmr/m/n/10.95 ([](\OML/cmm/m/it/10.95 s; a[]; b\OT1/cm
r/m/n/10.95 ) \OMS/cmsy/m/n/10.95 ^^R :\OML/cmm/m/it/10.95 X[] \OMS/cmsy/m/n/10
.95 _ []\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 s; a[]; b\OT1/cmr/m/n/10.95 ) \
OMS/cmsy/m/n/10.95 \ :\OML/cmm/m/it/10.95 Y[] \OMS/cmsy/m/n/10.95 6\OT1/cmr/m/n
/10.95 = \OMS/cmsy/m/n/10.95 ;\OT1/cmr/m/n/10.95 )

Underfull \hbox (badness 1158) in paragraph at lines 202--209
\OT1/ptm/m/n/10.95 Hence we have ei-ther al-ready proved that player 2 can en-s
ure the pre-de-ces-sor op-er-a-

Underfull \hbox (badness 1270) in paragraph at lines 202--209
\OT1/ptm/m/n/10.95 tor or $\OML/cmm/m/it/10.95 U[] \OT1/cmr/m/n/10.95 = \OML/cm
m/m/it/10.95 Z$ \OT1/ptm/m/n/10.95 in the end. If $\OML/cmm/m/it/10.95 U[]$ \OT
1/ptm/m/n/10.95 is $\OML/cmm/m/it/10.95 Z$ \OT1/ptm/m/n/10.95 in the end, then 
$\OML/cmm/m/it/10.95 Z$ \OT1/ptm/m/n/10.95 sat-is-fies the prop-erty

Underfull \hbox (badness 1297) in paragraph at lines 202--209
\OT1/ptm/m/n/10.95 used in the pre-vi-ous cases of $\OML/cmm/m/it/10.95 U[]$ \O
T1/ptm/m/n/10.95 (the proof of part a), and then as in the pre-vi-ous
[50])) [51]
Underfull \hbox (badness 6961) in paragraph at lines 1073--1094
[]\OT1/ptm/m/it/10.95 (Second in-clu-sion: $[][]\OT1/cmr/m/n/10.95 ([]\OML/cmm/
m/it/10.95 ; []; \OT1/cmr/m/n/10.95 ^^H) \OMS/cmsy/m/n/10.95 ^^R [][]\OT1/cmr/m
/n/10.95 ([]\OML/cmm/m/it/10.95 ; M; \OT1/cmr/m/n/10.95 ^^H)$\OT1/ptm/m/it/10.9
5 ). \OT1/ptm/m/n/10.95 We now show that
[52]) (./main.bbl [53] [54]) [55] (./main.aux)

LaTeX Warning: There were undefined references.

 )
(see the transcript file for additional information)
Output written on main.dvi (55 pages, 310768 bytes).
Transcript written on main.log.
This is pdfeTeXk, Version 3.141592-1.21a-2.2 (Web2C 7.5.4)
 file:line:error style messages enabled.
 %&-line parsing enabled.
entering extended mode
(./main.tex
LaTeX2e <2003/12/01>
Babel <v3.8d> and hyphenation patterns for american, french, german, ngerman, b
ahasa, basque, bulgarian, catalan, croatian, czech, danish, dutch, esperanto, e
stonian, finnish, greek, icelandic, irish, italian, latin, magyar, norsk, polis
h, portuges, romanian, russian, serbian, slovak, slovene, spanish, swedish, tur
kish, ukrainian, nohyphenation, loaded.
(/usr/share/texmf/tex/latex/base/article.cls
Document Class: article 2004/02/16 v1.4f Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size11.clo))
(/usr/share/texmf/tex/latex/base/latexsym.sty)
(/usr/share/texmf/tex/latex/amsmath/amstext.sty
(/usr/share/texmf/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf/tex/latex/amsfonts/amssymb.sty
(/usr/share/texmf/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf/tex/latex/preprint/fullpage.sty) (./epsfig.sty
Document style option `epsfig', v1.20 <26.1.94> (edited by SPQR)
(/usr/share/texmf/tex/generic/epsf/epsf.tex
This is `epsf.tex' v2.7k <10 July 1997>
)) (./eepic.sty
Extension to Epic and LaTeX. Version 1.1e - Released Dec 21, 1999
) (./gastex.sty (/usr/share/texmf/tex/latex/tools/calc.sty)
(/usr/share/texmf/tex/latex/graphics/trig.sty)) (./luca.sty)
(/usr/share/texmf/tex/latex/psnfss/times.sty) (./main.aux)
(/usr/share/texmf/tex/latex/psnfss/ot1ptm.fd)
(/usr/share/texmf/tex/latex/base/ulasy.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf/tex/latex/amsfonts/umsb.fd)
(/usr/share/texmf/tex/latex/psnfss/ot1pcr.fd) [1] [2] [3]

LaTeX Warning: Reference `examp-counter-almost' on page 4 undefined on input li
ne 566.

[4] (./definitions.tex (/usr/share/texmf/tex/latex/psnfss/omsptm.fd)
Underfull \hbox (badness 1783) in paragraph at lines 93--100
\OT1/ptm/b/n/10.95 Equivalent game struc-tures. \OT1/ptm/m/n/10.95 Given two ga
me struc-tures $\OMS/cmsy/m/n/10.95 G[] \OT1/cmr/m/n/10.95 = \OMS/cmsy/m/n/10.9
5 h\OML/cmm/m/it/10.95 S; []; \OT1/cmr/m/n/10.95 ^^@[]\OML/cmm/m/it/10.95 ; \OT
1/cmr/m/n/10.95 ^^@[]\OML/cmm/m/it/10.95 ; ^^N[]\OMS/cmsy/m/n/10.95 i$ \OT1/ptm
/m/n/10.95 and $\OMS/cmsy/m/n/10.95 G[] \OT1/cmr/m/n/10.95 =
[5] [6]
Underfull \hbox (badness 3229) in paragraph at lines 352--358
[]\OT1/ptm/m/n/10.95 Given a set $\OML/cmm/m/it/10.95 U \OMS/cmsy/m/n/10.95 ^^R
 \OML/cmm/m/it/10.95 S$ \OT1/ptm/m/n/10.95 we use usual LTL no-ta-tions $\U/las
y/m/n/10.95 2\OML/cmm/m/it/10.95 U; \U/lasy/m/n/10.95 3\OML/cmm/m/it/10.95 U; \
U/lasy/m/n/10.95 23\OML/cmm/m/it/10.95 U$ \OT1/ptm/m/n/10.95 and $\U/lasy/m/n/1
0.95 32\OML/cmm/m/it/10.95 U$ \OT1/ptm/m/n/10.95 to de-note
[7] [8]) (./pure.tex [9] [10] [11]
Underfull \hbox (badness 4096) in paragraph at lines 231--248
\OT1/ptm/b/n/10.95 Computation of $[][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 
U; M; \OT1/cmr/m/n/10.95 ^^H)$\OT1/ptm/b/n/10.95 . \OT1/ptm/m/n/10.95 It fol-lo
ws from Propo-si-tion 2[] that the com-pu-ta-tion of
(./big-proof1.tex [12] [13] [14]
Underfull \hbox (badness 2111) in paragraph at lines 230--236
[]\OT1/ptm/m/it/10.95 Observe that if the pred-i-cate $[][]\OT1/cmr/m/n/10.95 (
\OML/cmm/m/it/10.95 Y[]\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m/it/10.95 is re-moved fr
om the pre-de-ces-sor op-er-a-tor

Underfull \hbox (badness 10000) in paragraph at lines 230--236
[][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X[]\OT1/cmr/
m/n/10.95 )$ \OT1/ptm/m/it/10.95 (resp. $[][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/
10.95 i; Y[]; X[]; [] ; Y[]; X[]; Y[]\OT1/cmr/m/n/10.95 )$\OT1/ptm/m/it/10.95 )
,

Underfull \hbox (badness 10000) in paragraph at lines 230--236
\OT1/ptm/m/it/10.95 then we ob-tain the op-er-a-tor $[][]\OT1/cmr/m/n/10.95 (\O
ML/cmm/m/it/10.95 i \OMS/cmsy/m/n/10.95 ^^@ \OT1/cmr/m/n/10.95 1\OML/cmm/m/it/1
0.95 ; X[]; Y[]; [] ; X[]; Y[]; X[]\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m/it/10.95 (r
esp.

Overfull \hbox (4.46823pt too wide) detected at line 272
\OML/cmm/m/it/10.95 ^^WY[]:^^VX[]:^^WY[]:^^VX[]: [] ^^WY[]:^^VX[]:^^WY[]: []
[15]
Overfull \hbox (12.87668pt too wide) detected at line 306
\OML/cmm/m/it/10.95 ^^VY[]:^^WX[]:^^VY[]:^^WX[]: [] ^^VY[]:^^WX[]:^^VY[]: []
[16] [17] [18] [19]
Overfull \hbox (21.4319pt too wide) detected at line 717
[]

Underfull \hbox (badness 1675) in paragraph at lines 726--730
[]  []\OT1/ptm/m/it/10.95 For a par-ity func-tion $\OML/cmm/m/it/10.95 p \OT1/c
mr/m/n/10.95 : \OML/cmm/m/it/10.95 S \OMS/cmsy/m/n/10.95 7! \OT1/cmr/m/n/10.95 
[0\OML/cmm/m/it/10.95 ::\OT1/cmr/m/n/10.95 2\OML/cmm/m/it/10.95 n\OT1/cmr/m/n/1
0.95 ]$\OT1/ptm/m/it/10.95 , and for all $\OML/cmm/m/it/10.95 T \OMS/cmsy/m/n/1
0.95 ^^R \OML/cmm/m/it/10.95 S$\OT1/ptm/m/it/10.95 , we have $\OML/cmm/m/it/10.
95 W \OMS/cmsy/m/n/10.95 ^^R
[20] [21]
Overfull \hbox (2.68309pt too wide) detected at line 865
\OML/cmm/m/it/10.95 ^^WX[]:^^VY[]:^^WX[]: [] ^^VY[]:^^WX[]:^^VY[]: []
[22]
Overfull \hbox (8.2834pt too wide) detected at line 990
\OML/cmm/m/it/10.95 W \OT1/cmr/m/n/10.95 = \OML/cmm/m/it/10.95 ^^VX[]:^^WY[]:^^
VX[]: [] ^^WY[]:^^VX[] [] :
[23] [24]
Overfull \hbox (8.098pt too wide) detected at line 1159
\OML/cmm/m/it/10.95 ^^VY[]:^^WX[]:^^VY[]:^^WX[]: [] ^^VY[]:^^WX[] []
[25] [26] [27]
Overfull \hbox (8.098pt too wide) detected at line 1321
\OML/cmm/m/it/10.95 ^^VY[]:^^WX[]:^^VY[]:^^WX[]: [] ^^VY[]:^^WX[] []
[28] [29] (./dual-pre-uniform.tex
Underfull \hbox (badness 10000) in paragraph at lines 26--32
[]\OT1/ptm/m/it/10.95 For all $\OML/cmm/m/it/10.95 s \OMS/cmsy/m/n/10.95 2 \OML
/cmm/m/it/10.95 S$\OT1/ptm/m/it/10.95 , if $\OML/cmm/m/it/10.95 s \OMS/cmsy/m/n
/10.95 2 [][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X[]
\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m/it/10.95 (resp. $\OML/cmm/m/it/10.95 s \OMS/cm
sy/m/n/10.95 2

Underfull \hbox (badness 10000) in paragraph at lines 26--32
[][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X[]; Y[]\OT1
/cmr/m/n/10.95 )$\OT1/ptm/m/it/10.95 ), then there ex-ists uni-form dis-tri-bu-


Underfull \hbox (badness 10000) in paragraph at lines 26--32
\OT1/ptm/m/it/10.95 tion $\OML/cmm/m/it/10.95 ^^X[]$ \OT1/ptm/m/it/10.95 to wit
-ness that $\OML/cmm/m/it/10.95 s \OMS/cmsy/m/n/10.95 2 [][]\OT1/cmr/m/n/10.95 
(\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X[]\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m
/it/10.95 (resp. $\OML/cmm/m/it/10.95 s \OMS/cmsy/m/n/10.95 2
[30] [31] [32])) [33] [34]
Underfull \hbox (badness 6842) in paragraph at lines 514--519
[] \OT1/ptm/b/n/10.95 ($[][]\OT1/cmr/m/n/10.95 ([]\OML/cmm/m/it/10.95 ; []; \OT
1/cmr/m/n/10.95 ^^H) \U/msb/m/n/10.95 ( [][]\OT1/cmr/m/n/10.95 ([]\OML/cmm/m/it
/10.95 ; []; \OT1/cmr/m/n/10.95 ^^H)$\OT1/ptm/b/n/10.95 ).  []\OT1/ptm/m/n/10.9
5 We show with an ex-am-ple that
[35]) (./limit-finite.tex [36] [37]
Overfull \hbox (13.0226pt too wide) in paragraph at lines 342--345
 [] 
[38] (./big-proof2.tex [39] [40] [41]
Underfull \hbox (badness 3668) in paragraph at lines 196--201
[]\OT1/ptm/m/it/10.95 Observe that if we rule out the pred-i-cate $[][]\OT1/cmr
/m/n/10.95 (\OML/cmm/m/it/10.95 X[]; Y[]\OT1/cmr/m/n/10.95 )$ \OT1/ptm/m/it/10.
95 the pre-de-ces-sor op-er-a-tor

Underfull \hbox (badness 3701) in paragraph at lines 196--201
\OT1/ptm/m/it/10.95 then we ob-tain the sim-pler pre-de-ces-sor op-er-a-tor $[]
[]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 i; X[]; Y[]; [] ; Y[]; X[]\OT1/cmr/m/
n/10.95 )$ \OT1/ptm/m/it/10.95 (resp.
(./formal-limit-pre.tex [42] [43]) [44] [45]
Underfull \hbox (badness 10000) in paragraph at lines 392--401
\OT1/ptm/b/n/10.95 Claim. \OT1/ptm/m/n/10.95 We show that for $\OML/cmm/m/it/10
.95 X[] \OMS/cmsy/m/n/10.95 ^^R \OML/cmm/m/it/10.95 X[] \OMS/cmsy/m/n/10.95 ^^R
 \OML/cmm/m/it/10.95 Y[] \OMS/cmsy/m/n/10.95 ^^R \OML/cmm/m/it/10.95 Y[]$ \OT1/
ptm/m/n/10.95 we have
[46] [47] (./gen.tex
Overfull \hbox (6.37802pt too wide) detected at line 28
[]
[48]
Overfull \hbox (18.19014pt too wide) in paragraph at lines 58--86
[]\OT1/ptm/m/n/10.95 We first show that if $[][] \OT1/cmr/m/n/10.95 = ^^@[](\OM
L/cmm/m/it/10.95 s\OT1/cmr/m/n/10.95 )$\OT1/ptm/m/n/10.95 , then $\OML/cmm/m/it
/10.95 s \OMS/cmsy/m/n/10.95 2 [][]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 Y[];
 X[]\OT1/cmr/m/n/10.95 )  []  [][](\OML/cmm/m/it/10.95 i; Y[]; X[]; [] ; Y[]; X
[]\OT1/cmr/m/n/10.95 )$\OT1/ptm/m/n/10.95 .
[49]
Overfull \hbox (13.0751pt too wide) detected at line 186
[]\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 s; a[]; b\OT1/cmr/m/n/10.95 ) \OMS/cm
sy/m/n/10.95 ^^R :\OML/cmm/m/it/10.95 X[] \OMS/cmsy/m/n/10.95 ^ 9\OT1/cmr/m/n/1
0.95 0 \OMS/cmsy/m/n/10.95 ^^T \OML/cmm/m/it/10.95 j \OMS/cmsy/m/n/10.95 ^^T \O
ML/cmm/m/it/10.95 i:\OT1/cmr/m/n/10.95 ([](\OML/cmm/m/it/10.95 s; a[]; b\OT1/cm
r/m/n/10.95 ) \OMS/cmsy/m/n/10.95 ^^R :\OML/cmm/m/it/10.95 X[] \OMS/cmsy/m/n/10
.95 _ []\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 s; a[]; b\OT1/cmr/m/n/10.95 ) \
OMS/cmsy/m/n/10.95 \ :\OML/cmm/m/it/10.95 Y[] \OMS/cmsy/m/n/10.95 6\OT1/cmr/m/n
/10.95 = \OMS/cmsy/m/n/10.95 ;\OT1/cmr/m/n/10.95 )

Underfull \hbox (badness 1158) in paragraph at lines 202--209
\OT1/ptm/m/n/10.95 Hence we have ei-ther al-ready proved that player 2 can en-s
ure the pre-de-ces-sor op-er-a-

Underfull \hbox (badness 1270) in paragraph at lines 202--209
\OT1/ptm/m/n/10.95 tor or $\OML/cmm/m/it/10.95 U[] \OT1/cmr/m/n/10.95 = \OML/cm
m/m/it/10.95 Z$ \OT1/ptm/m/n/10.95 in the end. If $\OML/cmm/m/it/10.95 U[]$ \OT
1/ptm/m/n/10.95 is $\OML/cmm/m/it/10.95 Z$ \OT1/ptm/m/n/10.95 in the end, then 
$\OML/cmm/m/it/10.95 Z$ \OT1/ptm/m/n/10.95 sat-is-fies the prop-erty

Underfull \hbox (badness 1297) in paragraph at lines 202--209
\OT1/ptm/m/n/10.95 used in the pre-vi-ous cases of $\OML/cmm/m/it/10.95 U[]$ \O
T1/ptm/m/n/10.95 (the proof of part a), and then as in the pre-vi-ous
[50])) [51]
Underfull \hbox (badness 6961) in paragraph at lines 1073--1094
[]\OT1/ptm/m/it/10.95 (Second in-clu-sion: $[][]\OT1/cmr/m/n/10.95 ([]\OML/cmm/
m/it/10.95 ; []; \OT1/cmr/m/n/10.95 ^^H) \OMS/cmsy/m/n/10.95 ^^R [][]\OT1/cmr/m
/n/10.95 ([]\OML/cmm/m/it/10.95 ; M; \OT1/cmr/m/n/10.95 ^^H)$\OT1/ptm/m/it/10.9
5 ). \OT1/ptm/m/n/10.95 We now show that
[52]) (./main.bbl [53] [54]) [55] (./main.aux)

LaTeX Warning: There were undefined references.

 )
(see the transcript file for additional information)
Output written on main.dvi (55 pages, 310768 bytes).
Transcript written on main.log.

